Precise Mobile Manipulation of Small Everyday Objects

Many everyday mobile manipulation tasks require precise interaction with small objects, such as grasping a knob to open a cabinet or pressing a light switch. In this paper, we develop Servoing with Vision Models (SVM), a closed-loop framework that enables a mobile manipulator to tackle such precise tasks involving the manipulation of small objects. SVM uses state-of-the-art vision foundation models to generate 3D targets for visual servoing to enable diverse tasks in novel environments. Naively doing so fails because of occlusion by the end-effector. SVM mitigates this using vision models that out-paint the end-effector, thereby significantly enhancing target localization. We demonstrate that aided by out-painting methods, open-vocabulary object detectors can serve as a drop-in module for SVM to seek semantic targets (e.g. knobs) and point tracking methods can help SVM reliably pursue interaction sites indicated by user clicks. We conduct a large-scale evaluation spanning experiments in 10 novel environments across 6 buildings including 72 different object instances. SVM obtains a 71% zero-shot success rate on manipulating unseen objects in novel environments in the real world, outperforming an open-loop control method by an absolute 42% and an imitation learning baseline trained on 1000+ demonstrations also by an absolute success rate of 50%.

==> 1-intro-v4.tex <==
\section{Introduction (v2)}
\seclabel{intro-v2}















==> 6-cover.tex <==
\newpage
\section*{Cover Letter}

\noindent Dear Prof. Tamim Asfour,

We are submitting our work, ``Precise Mobile Manipulation of Small Everyday Objects'' to RA-L. This work presents a novel methodology that enables precise and generalizable mobile manipulation in the real world, achieving strong performance and outperforming established baselines. 

An early version of this work, titled ``A Training-Free Framework for Precise Mobile Manipulation of Small Everyday Objects,'' (submission number 25-0499) was submitted in February 2025. We received a number of encouraging comments at that time. For example, Reviewer 414991 noted that our system ``shows good success at performing the defined tasks'' and ``has the potential to be really strong for a wide variety of tasks.'' Reviewer 415017 commented that the presentation was ``clear and easy to follow.'' Reviewer 415015 highlighted that our approach ``integrates visual servoing and modern perception methods for precise and generalizable robotic manipulation,'' and further commended the paper for ``offering detailed and clear descriptions of the proposed approach, enhancing reproducibility and facilitating future research efforts by the broader robotics community.''

The meta-review summarized the main concerns as relating to: (a) the number of evaluations, (b) comparison with baselines, (c) task selection, and (d) limitations of the proposed method. Since then, we have substantially revised the work to address these points. Specifically:

\begin{itemize}[leftmargin=*]
    \item \textbf{Number of evaluations and evaluation diversity.} 
    Reviewers expressed concern that our original submission had too few trials per task and limited diversity across environments, which could affect the reliability of the reported results. To address this, we have substantially expanded our evaluation. Specifically, we increased the number of unique objects from 28 to 72, and added three new previously unseen environments as well as two additional buildings for a total of $10$ environments across $6$ buildings. The number of trials has also been increased: Table~2 (comparison with RUM) now includes $3\times$ the number of trials, and Table~1 has $1.5\times$ the number of trials compared to the original manuscript. Additionally, to assess repeatability within a single environment and object, we open the same drawer $5\times$ from distinct starting locations and find that all $5$ trials succeed. These changes provide a much stronger empirical basis for the reported results, demonstrating consistency across a broader range of objects, settings, and repetitions. To better illustrate the expanded diversity, we have added a figure in the main paper showing the variety of objects and environments, and an additional slide in the supplementary video.



    \item \textbf{Comparison with baselines.} 
    Reviewers raised concerns that our comparison to RUM may not have been entirely fair, due to differences in task domains, hardware setups, and evaluation details. In the revision, we have strengthened the fairness and transparency of this comparison. Specifically: (a) we used RUM's exact hardware setup and starting configuration as specified for evaluation; (b) we evaluated on both handles (the setting RUM was trained on) and knobs, demonstrating improvements in both cases; and (c) we aided RUM by conducting three trials with varying starting heights of the end-effector and reporting its best result, since its method requires the initial height as input whereas ours does not. In addition, we tripled the number of trials (from 10 to 30) across 6 buildings to provide a broader and more reliable basis for comparison. These steps ensure that the reported improvements are substantial.



    \item \textbf{Task selection.} 
    Reviewers suggested that our evaluation could be expanded,
    for example by including visual-servoing-based grasping, and also noted that our framework primarily addresses precise reaching and alignment, with task completion relying on motion primitives. In the revision, we have broadened the task set. Our evaluation now spans six distinct mobile manipulation tasks across three families: (a) grasping knobs to open drawers and cabinets, (b) grasping handles to open cabinets, and (c) pushing interactions such as buttons, switches, and books. Importantly, the articulated object tasks explicitly require {\it grasping} the knob or handle before execution of the primitive, thereby directly evaluating the contribution of our servoing framework to successful grasping. In addition, we expanded the diversity of pushing tasks to include real-world scenarios such as pressing thermostat buttons and flipping extension-cord switches. In summary, the six tasks we report results on demonstrate that our method supports precise grasping as well as reliable execution in realistic and diverse settings. While any robotics paper could be improved by adding more tasks, we believe our task diversity is commensurate with typical robotics papers.

    \item \textbf{Limitations.} 
    Reviewers requested a clearer discussion of the limitations and failure modes of our approach. In the revision, we include this explicitly. 
    Specifically, we find that across 20 failures of \name, 35\% were perception errors and 65\% were execution errors (see \figref{waterfall_chart}). Within perception, mis-detections were surprisingly the dominant failure mode, despite using a vision foundation model. Within execution, insufficient precision was the dominant cause of failure. 
    This suggests that future work should focus on strengthening eye-in-hand perception models and improving precise control under limited degrees of freedom.

\end{itemize}









\noindent Next, we address each reviewer concern below.

\subsection{Review414991 (Reviewer1)}

\subsubsection{Number of evaluations}
\textit{All the real world evaluations are done
between 2-7 times, where 7 is the maximum number of different
environments. This makes me thing that there was only one evaluation
per environment, which is concerning because even on the same
environment, based on different starting location, the success rate can
vary especially for neural methods. Therefore, only one evaluation per
environment is surprisingly lackluster.}

\textbf{Response:} To address this, we have substantially expanded our evaluation. The number of trials has been increased: Table~2 (comparison with RUM) now includes $3\times$ the number of trials, and Table~1 has $1.5\times$ the number of trials compared to the original manuscript. 
Additionally, to assess repeatability within a single environment and object, we open the same drawer $5\times$ from distinct starting locations and find that all $5$ trials succeed.
These changes provide a much stronger empirical basis for the reported results, demonstrating consistency across a broader range of objects and settings.
\vspace{0.5cm}

\subsubsection{Evaluation environment diversity}
\textit{For many of the evaluations, the
environment seems to be the same with slightly different knob or
handle, replaced by the authors. It does not capture the diversity seen
in real world cabinets properly, and may bias the results towards
particular environments.}

\textbf{Response:} To address this, we have  added three new previously unseen environments as well as two additional buildings for a total of 10 unseen environments from 6 buildings. We have also increased the number of unique objects from 28 to 72. To better illustrate the expanded diversity, we have added a figure in the main paper showing the variety of objects and environments, and an additional slide in the supplementary video.
\vspace{0.5cm}

\subsubsection{Selection of tasks}
\textit{While the five tasks selected cover variety of
different types of motion, the authors can easily expand upon it by,
for example, using a visual servoing based grasping. That would be a
very useful evaluation for practitioners in the field.}

\textbf{Response:} To address this, we have broadened the task set. Our evaluation now spans six distinct mobile manipulation tasks across three families: (a) grasping knobs to open drawers and cabinets, (b) grasping handles to open cabinets, and (c) pushing interactions such as buttons, switches, and books. Importantly, the articulated object tasks explicitly require grasping the knob or handle before execution of the primitive, thereby directly evaluating the contribution of our servoing framework to successful grasping. In addition, we expanded the diversity of pushing tasks to include real-world scenarios such as pressing thermostat buttons and flipping extension-cord switches. As a whole, the six tasks we report results on demonstrate that our method supports precise grasping as well as reliable execution in realistic and diverse settings.
\vspace{0.5cm}

\subsubsection{Lack of clarity on limitations}
\textit{While the authors show different
cases this system may work, it is not clear where it doesn't. For
example, there are no cases of doors with horizontal handles (all
horizontal handles were replaced by knobs) but there are no clarity on
if this is an inherent limitation of the system or just incidental.}

\textbf{Response:} To address this, we include a discussion of the limitations of our system in the main paper. In summary, major limitations include: (a) high latency of the system, (b) reliance on depth, and (c) the hand-crafted nature of the task decomposition. Furthermore, the lack of horizontal handles is just incidental, and not a fundamental limitation of the system.

\vspace{0.5cm}

\subsubsection{Poor baseline evaluation}
\textit{The authors compare with RUMs, which are
trained on large demonstration datasets, but does not mention that the
evaluated models were explicitly not targeted towards or trained on
doors and drawers with knobs, which was mentioned in the limitation.
Therefore, the comparison, which does not mention this limitation in
the paper, seems unfair out of the box.}

\textbf{Response:} We clarify the fairness of our comparison to RUM. Specifically: (a) we used RUM's exact hardware setup and starting configuration as specified for evaluation; (b) we evaluated on both handles (the setting RUM was trained on) and knobs, demonstrating improvements in both cases; and (c) we aided RUM by conducting three trials with varying starting heights of the end-effector and reporting its best result, since its method requires the initial height as input whereas ours does not. In addition, we tripled the number of trials (from 10 to 30) across 6 buildings to provide a broader and more reliable basis for comparison. These steps ensure that the reported improvements are both fair and substantial.
\vspace{0.5cm}

\subsubsection{Proper breakdown of failure modes}
\textit{Since the proposed system, SVM,
is modular, there is a lot of value in understanding which module is
failing in the failure cases. Therefore, adding a waterfall chart or a
sankey diagram would improve the analysis immensely.}

\textbf{Response:} To address this, we include a dicussion of the failure modes of our method in the main paper. Specifically, we find that across 20 failures of \name, 35\% were perception errors and 65\% were execution errors (see \figref{waterfall_chart}). Within perception, mis-detections were surprisingly the dominant failure mode, despite using a vision foundation model. Within execution, insufficient precision was the dominant cause of failure. 
This suggests that future work should focus on strengthening eye-in-hand perception models and improving precise control under limited degrees of freedom.
\vspace{0.5cm}








\subsection{Review415015 (Reviewer2)}

\subsubsection{Number of evaluations}
\textit{Given the simplicity and training-free nature of the proposed
approach, the experimental evaluation could be more extensive.
Specifically, the small number of trialsóonly two trials per task for
user-clicked targets in Table I, and three to four trials per task in
Table IIólimits the statistical significance and reliability of the
presented results.}

\textbf{Response:} To address this, we have substantially expanded our evaluation. The number of trials has been increased: Table~2 (comparison with RUM) now includes $3\times$ the number of trials, and Table~1 has $1.5\times$ the number of trials compared to the original manuscript. 
Additionally, to assess repeatability within a single environment and object, we open the same drawer $5\times$ from distinct starting locations and find that all $5$ trials succeed.
These changes provide a much stronger empirical basis for the reported results, demonstrating consistency across a broader range of objects and settings.
\vspace{0.5cm}

\subsubsection{Limitation of methodology}
\textit{The framework as described primarily addresses the problem of
precise reaching or alignment with target objects rather than providing
a complete solution for general mobile manipulation. Achieving
different manipulation tasks still relies on predefined, task-specific
motion primitives, potentially limiting broader applicability.}

\textbf{Response:} Yes, the framework tackles a finite number of tasks, and is by no means \textit{a complete solution for general mobile manipulation}. Nonetheless, we argue that our framework enables robots to perform a wide variety of useful tasks (ranging from opening articulated objects to pushing books into bookshelves), and do so on \textit{completely unseen objects} in \textit{completely unseen environments} in a zero-shot manner, something imitation learning-based approaches significantly struggle with.
While the motion primitives are predefined in this version of the work, it may be possible to obtain these from LLMs or from demonstrations, which we leave to future work.
\vspace{0.5cm}

\subsubsection{Evaluation environment diversity}
\textit{Considering the reliance on advanced vision models, the evaluation
lacks sufficient diversity in visual scenarios and backgrounds. A more
thorough assessment across varied visual conditions (e.g., lighting
variations, cluttered environments, challenging textures) would better
reflect the robustness and limitations of these perception models.}

\textbf{Response:} To address this, we have added three new previously unseen environments as well as two additional buildings for a total of 10 unseen environments from 6 buildings. We have also increased the number of unique objects from 28 to 72. To better illustrate the expanded diversity, we have added a figure in the main paper showing the variety of objects and environments, and an additional slide in the supplementary video.
\vspace{0.5cm}

\subsubsection{Poor baseline comparison}
\textit{The presented comparison against the RUM baseline model is not entirely fair, as differences exist between the experimental setups, particularly regarding the type of end-effector and camera sensor used. These differences could unfairly disadvantage RUM and potentially influence the observed performance gap.}

\textbf{Response:} 
Both the original RUM paper and our reproduction observe a decent success rate with the RUM hardware, showing that this end-effector and camera configuration is capable of successful interaction with articulated objects. Furthermore, the dominant RUM failures we observe arise from the model closing the grippers at an incorrect 3D location, i.e. an algorithmic issue rather than a hardware limitation. Finally, it is a system-level comparison: RUM is the state-of-the-art system for this task that {\it chose} to use this custom hardware to get the best performance for their system, \vs our method that just uses commodity hardware that comes with the Stretch. Specifically, the RUM paper discusses the deliberate choice of using an iPhone Pro (\vs Intel RGB-D cameras in earlier efforts~\cite{song2020grasping}) to ease scaling up of data collection, and Shafiullah \etal~\cite{shafiullah2023bringing} (that designed v1 of the Stick used in RUM) notes ``[small cylindrical tips] helps our system manipulate finer objects, such as door and drawer handles, without getting stuck or blocked.'' We were careful to (a) use RUM's exact hardware setup and starting configuration as specified for evaluation and (b) evaluate on drawer and cabinet handles, the tasks that RUM was specifically trained for. Furthermore, we aided RUM by conducting three trials with varying starting heights of the end-effector and reporting its {\it best} result. 
Finally, we more than doubled the number of trials (from 10 to 30) across 6 buildings to provide a broader and more reliable basis for comparison. These steps ensure that the reported improvements are both fair and substantial.
\vspace{0.5cm}

\subsection{Review415017 (Reviewer3)}

\subsubsection{Positioning of paper}
\textit{The positioning of the paper’s argument is somewhat unclear. It claims
that the primary challenge in mobile manipulation is “reaching an
accurate pre-task pose” for small target objects. The experimental task
setting, which relies on motion primitives across all tasks, seems to
support this argument. However, the experiment only tests one type of
pre-task pose (horizon grasping) with no variation in translation or
orientation, which appears to contradict the initial claim.}

\textbf{Response:} We clarify that there is variation in the pre-task pose across the different tasks, and even across different trials. Specifically, the pre-task pose when opening a cabinet, which is determined by MOSART~\cite{gupta2024opening}, is vastly different from the pre-task pose when trying to push a light button (which the base position and end-effector pose is arbitrarily varied in front of the object). As a result, there is a significant amount of variation in the translation and orientation of the pre-task pose, and reliably getting from an arbitrary pre-task pose to the desired site of interaction is a challenge we provide a methodology for.
\vspace{0.5cm}

\subsubsection{Necessity of closing the loop}
\textit{Building on the previous point, if the problem is truly just about
“accurately reaching a specific point” (such as the center of a handle
or button) in a fixed-base setting, it’s unclear why closed-loop
execution is necessary. Can’t the grasping point simply be computed and
reached by reprojecting to 3D space using a calibrated camera?}

\textbf{Response:} We clarify that Table I includes a comparison to the open-loop baseline that the reviewer proposes. Specifically, MOSART~\cite{gupta2024opening} does open-loop control using the head camera from 1.5m away, and our additional "Open-Loop (Eye-in-Hand)" baseline does open-loop control from the pre-task pose using the eye-in-hand camera. We find that the open-loop methodologies work reasonably well for low-precision tasks (e.g. grasping handles), but struggle with high-precision tasks (e.g. grasping knobs), where our closed-loop approach excels. This may be due to a combination of both imperfect camera calibration, as well as the use of a low-DoF commodity mobile manipulator with limited precision.
\vspace{0.5cm}

\subsubsection{Selection of baselines}
\textit{The selection of baselines is also questionable. The authors argue that
their approach outperforms RUM due to its use of an object-centric
representation (such as object detection or point tracking). However,
this overlooks the fact that imitation learning methods [1, 2] can also
leverage this kind of information effectively.}

\textbf{Response:} 
Although an IL baseline could be augmented with object-centric inputs, our newly extended experiments with RUM suggest this is not the primary limitation in our setting. The dominant failure mode we observe for RUM is hovering: the policy attends to the correct region but exhibits oscillatory, indecisive actions, rather than selecting the wrong object. Wrong-object errors are rare, in part because our tasks contain few plausible distractors (see \figref{diversity}). Thus, merely cropping around the object does not address the key issue: stabilizing control under distribution shifts due to minor pose/appearance changes. \name's gains instead come from coupling robust, pre-trained vision foundation models (for reliable detection/feature tracking under occlusion and lighting changes) with closed-loop servoing, which continuously corrects approach errors and mitigates dithering/compounding-error behavior typical of open-loop IL—regardless of whether inputs are full-image or object-centric.

\vspace{0.5cm}

\subsubsection{Limited task suite}
\textit{Additionally, the task suite is somewhat limited for "mobile
manipulation of small everyday objects," as it focuses solely on
articulated objects and non-prehensile tasks, while lacking common task
types like general pick-and-place or object reorientation.}

\textbf{Response:} We have broadened the task set. Our evaluation now spans six distinct mobile manipulation tasks across three families: (a) grasping knobs to open drawers and cabinets, (b) grasping handles to open cabinets, and (c) pushing interactions such as buttons, switches, and books. In addition, we expanded the diversity of pushing tasks to include real-world scenarios such as pressing thermostat buttons and flipping extension-cord switches. As a whole, the six tasks we report results on demonstrate that our method supports precise grasping as well as reliable execution in realistic and diverse settings.
\vspace{0.5cm}

\noindent Taken together, these revisions directly address the reviewers’ feedback and significantly strengthen both the empirical evaluation and the clarity of the paper. We believe that the resulting manuscript presents a compelling case for our novel methodology which enables precise and generalizable mobile manipulation, and will be of interest to a broad robotics audience. Thank you for your time and consideration.

